Sparse and Dense Approaches for the Full-rank Retrieval of Responses for Dialogues

Ranking responses for a given dialogue context is a popular benchmark in which the setup is to re-rank the ground-truth response over a limited set of $n$ responses, where $n$ is typically 10. The predominance of this setup in conversation response ranking has lead to a great deal of attention to building neural re-rankers, while the first-stage retrieval step has been overlooked. Since the correct answer is always available in the candidate list of $n$ responses, this artificial evaluation setup assumes that there is a first-stage retrieval step which is always able to rank the correct response in its top-$n$ list. In this paper we focus on the more realistic task of full-rank retrieval of responses, where $n$ can be up to millions of responses. We investigate both dialogue context and response expansion techniques for sparse retrieval, as well as zero-shot and fine-tuned dense retrieval approaches. Our findings based on three different information-seeking dialogue datasets reveal that a learned response expansion technique is a solid baseline for sparse retrieval. We find the best performing method overall to be dense retrieval with intermediate training, i.e. a step after the language model pre-training where sentence representations are learned, followed by fine-tuning on the target conversational data. We also investigate the intriguing phenomena that harder negatives sampling techniques lead to worse results for the fine-tuned dense retrieval models. The code and datasets are available at https://github.com/Guzpenha/transformer_rankers/tree/full_rank_retrieval_dialogues.

==> tables/diff_loss_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[]
\caption{Effectiveness of fine-tuned dense retrieval models when using different loss functions for each negative sampling procedures from Table~\ref{table:main_table_results}. We observe the same phenomena of decreasing effectiveness for better negative sampling methods with different loss functions. Bold indicates the highest value within different negative sampling methods for the same setting.}
\label{table:diff_loss}
\begin{tabular}{@{}lrrrrrrr@{}}
\toprule
\textbf{} & \textbf{} & \multicolumn{2}{c}{\textbf{\mantis{}}} & \multicolumn{2}{c}{\textbf{\msdialog{}}} & \multicolumn{2}{c}{\textbf{\ubuntu{}}} \\ \midrule
\textbf{Loss} & \textbf{Negative Sampler} & \multicolumn{1}{l}{\textbf{R@1}} & \multicolumn{1}{l}{\textbf{R@10}} & \multicolumn{1}{l}{\textbf{R@1}} & \multicolumn{1}{l}{\textbf{R@10}} & \multicolumn{1}{l}{\textbf{R@1}} & \multicolumn{1}{l}{\textbf{R@10}} \\ \midrule
\multirow{3}{*}{MulNegRankLoss} & Random (0) & \textbf{0.130} & \textbf{0.307} & \textbf{0.168} & \textbf{0.387} & \textbf{0.050} & \textbf{0.128} \\
 & \bm{} (1a) & 0.112 & 0.271 & 0.128 & 0.316 & 0.027 & 0.087 \\
 & Bi-encoder (3e) & 0.065 & 0.146 & 0.144 & 0.306 & 0.018 & 0.051 \\ \midrule
\multirow{3}{*}{ContrastiveLoss} & Random (0) &  &  &  &  &  &  \\
 & \bm{} (1a) &  &  &  &  &  &  \\
 & Bi-encoder (3e) &  &  &  &  &  &  \\ \midrule
\multirow{3}{*}{TripletLoss} & Random (0) &  &  &  &  &  &  \\
 & \bm{} (1a) &  &  &  &  &  &  \\
 & Bi-encoder (3e) &  &  &  &  &  &  \\ \bottomrule
\end{tabular}
\end{table*}
